Subgraph Stationary Hardware-Software Inference Co-Design

A growing number of applications depend on Machine Learning (ML) functionality and benefits from both higher quality ML predictions and better timeliness (latency) at the same time. A growing body of research in computer architecture, ML, and systems software literature focuses on reaching better latency-accuracy tradeoffs for ML models. Efforts include compression, quantization, pruning, early-exit models, mixed DNN precision, as well as ML inference accelerator designs that minimize latency and energy, while preserving delivered accuracy. All of them, however, yield improvements for a single static point in the latency-accuracy tradeoff space. We make a case for applications that operate in dynamically changing deployment scenarios, where no single static point is optimal. We draw on a recently proposed weight-shared SuperNet mechanism to enable serving a stream of queries that uses (activates) different SubNets within this weight-shared construct. This creates an opportunity to exploit the inherent temporal locality with our proposed SubGraph Stationary (SGS) optimization. We take a hardware-software co-design approach with a real implementation of SGS in SushiAccel and the implementation of a software scheduler SushiSched controlling which SubNets to serve and what to cache in real-time. Combined, they are vertically integrated into SUSHI-an inference serving stack. For the stream of queries, SUSHI yields up to 25% improvement in latency, 0.98% increase in served accuracy. SUSHI can achieve up to 78.7% off-chip energy savings.

==> Plot/memory_bound_layer_shifting.tex <==
\begin{figure}[t]
    \centering
    \subfloat[WS-ResNet 50.\label{fig:memory_resnet50}]{{\includegraphics[width=0.48\columnwidth]{Plot/memory_boundness_shifting_across_compute_resnet50.pdf}}}
    \subfloat[WS-MobileNet V3.\label{fig:memory_mbv3}]{{\includegraphics[width=0.48\columnwidth]{Plot/memory_boundness_shifting_across_compute_mbv3.pdf}}}
    \vspace{-2mm}
    \caption{Ablation study of throughput}
    \label{fig:memory_bound_shifting}
    % \vspace{-3mm}
\end{figure}

==> Plot/memory_boundness_layer_shifting_off_chip_banwidth.tex <==
\begin{figure}[t]
    \centering
    \subfloat[WS-ResNet 50.\label{fig:memory_resnet50_off_chip_bandwidth}]{{\includegraphics[width=0.48\columnwidth]{Plot/memory_boundness_shifting_across_off_chip_bandwidth_resnet50.pdf}}}
    \subfloat[WS-MobileNet V3.\label{fig:memory_mbv3_off_chip_bandwidth}]{{\includegraphics[width=0.48\columnwidth]{Plot/memory_boundness_shifting_across_off_chip_bandwidth_mbv3.pdf}}}
    \vspace{-2mm}
    \caption{Ablation study of off-chip bandwidth}
    \label{fig:memory_bound_shifting_off_chip_bandwidth}
    % \vspace{-3mm}
\end{figure}

==> Plot/pb_SR_bonus.tex <==
\begin{figure}[t]
    \centering
    \subfloat[ResNet50.\label{fig:pb_resnet50}]{{\includegraphics[width=0.48\columnwidth]{Plot/PB_size_exploration_resnet50.pdf}}}
    \subfloat[MobV3.\label{fig:pb_mbv3}]{{\includegraphics[width=0.51\columnwidth]{Plot/PB_size_exploration_mbv3.pdf}}}
    \vspace{-4mm}
    \caption{Exploring PB size on latency reduction.}
    \label{fig:pb_shifting}
    \vspace{-3mm}
    % \vspace{-3mm}
\end{figure}

==> Plot/real_board_results.tex <==
\begin{figure}[t]
    \centering
    \subfloat[Latency Comparison \label{fig:real_board_latency}]{{\includegraphics[width=0.44\linewidth]{Plot/latency_comparison_VS_CPU.pdf}}} 
    \subfloat[Latency Power Comparison \label{fig:real_board_latency_power}]{{\includegraphics[width=0.56\linewidth]{Plot/Latency_Power_Comparison.pdf}}}
    \vspace{-2mm}
    \caption{Latency and power comparison for \Accel on ZCU 104 and Intel 10-th i7 processor.\payman{Jianming: Can you please unify figs 13 and 14. Part a is similar. the legend stil has fastswitch. we need two plots: one for each FPGA! }}
    \vspace{-3mm}
    \label{fig:real_board_results}
\end{figure}


==> Src_Tex/Outline.tex <==
\renewcommand{\labelenumii}{\arabic{enumi}.\arabic{enumii}}
\renewcommand{\labelenumiii}{\arabic{enumi}.\arabic{enumii}.\arabic{enumiii}}
\renewcommand{\labelenumiv}{\arabic{enumi}.\arabic{enumii}.\arabic{enumiii}.\arabic{enumiv}}

\begin{enumerate}
\item One
    \item Three point one
\item Two
\item Three
\begin{enumerate}
    \item Three point one
    \begin{enumerate}
    \item Three point one, point one
        \begin{enumerate}
        \item Three point one, point one, point one
        \item Three point one, point one, point two
        \end{enumerate}
    \end{enumerate}
\end{enumerate}
\item Four
\item Five
\end{enumerate}



==> tables/best_searched_results.tex <==
\begin{table}[!t]
    \centering
    \scriptsize
    \vspace{-2mm}
    \caption{Best SR Bonus Configurations}
    \begin{tabular}{cccc}
        \hline 
         Factor / Set Up & WS-ResNet 50 & WS-MobileNet V3   \\ \hline
         Throughput (TFLOPS)  & 27.65  & 22.12        \\
         Off-chip bandwidth (GB/s)  & 1.6 & 1.6       \\ 
         PB Size (MB) & 7.55 & 3.94                   \\ 
         SR Bonus (\%) & 32.55 & 33.62                \\ 
        common weights Size (MB) & 7.55 & 2.90            \\ 
         \hline
    \end{tabular}
    \label{tab:best_SR_Bonus}
\end{table}


==> tables/dse_design_space.tex <==
\begin{table}[!t]
    \centering
    \scriptsize
    \vspace{-2mm}
    \caption{Constraints of related factors for SR}
    \begin{tabular}{cc}
        \hline 
         Factor & Upper threshold              \\ \hline
         Throughput  & 100 TFlops (MAX in embedded group)~\cite{AI_Accel_survey}              \\
         Off-chip bandwidth  &  38 GB/s (DDR4 on Xilinx Alveo U280)    \\ 
         PB Size  & total sizes of common weights     \\ 
         \hline
    \end{tabular}
    \label{tab:dse_parameter_range}
\end{table}

